Differentiable Convex Polyhedra Optimization from Multi-view Images

This paper presents a novel approach for the differentiable rendering of convex polyhedra, addressing the limitations of recent methods that rely on implicit field supervision. Our technique introduces a strategy that combines non-differentiable computation of hyperplane intersection through duality transform with differentiable optimization for vertex positioning with three-plane intersection, enabling gradient-based optimization without the need for 3D implicit fields. This allows for efficient shape representation across a range of applications, from shape parsing to compact mesh reconstruction. This work not only overcomes the challenges of previous approaches but also sets a new standard for representing shapes with convex polyhedra.

==> table/tab3_runtime.tex <==
\begin{table}

\centering
\resizebox{\linewidth}{!}{%
\addtolength{\tabcolsep}{8pt} 
  \begin{tabular}{l ccccc cc cccc}
  \toprule  
  % \cmidrule(lr){2-5}
  % \cmidrule(lr){6-7}  
  % \cmidrule(lr){8-10}
  % \cmidrule(lr){11-13}
  % \cmidrule(lr){14-15}
  %   \cmidrule(lr){16-17}
   & \bf \#Convexes & 1 & 2 & 4 & 8 & 16 &  32 &  64 & 128 & 256 & 512  \\
  
  \midrule
  \bf \#Planes 8 & \bf Time(Sec)    & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 & 0.03 & 0.03 & 0.05 & 0.09\\
                 & \bf Memory (MB) & 0.5 & 0.5 & 0.5 & 0.5 & 0.8 & 0.8 & 0.8 & 1.0 &  1.8 & 3.0 \\
  \midrule
  \bf \#Planes 16 & \bf Time(Sec)    & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 & 0.03 & 0.04 & 0.06 & 0.1 & 0.16\\
                 & \bf Memory (MB) & 0.5 & 0.5 & 0.5 & 0.5 & 0.8 & 1.0 & 1.2 & 2.0 & 3.8  & 7.0\\
  \midrule
  \bf \#Planes 32 & \bf Time(Sec)    & 0.02 & 0.02 & 0.02 & 0.02 & 0.03 & 0.04 & 0.05 & 0.1 & 0.17 & 0.33\\
                 & \bf Memory (MB) & 0.5 & 0.8 & 0.8 & 0.8 & 1.0 & 1.2 & 2.2 & 3.8 & 7.5 & 14.5\\
  \midrule
  \bf \#Planes 64 & \bf Time(Sec)    & 0.02 & 0.02 & 0.02 & 0.03 & 0.04 & 0.06 & 0.1 & 0.17 & 0.33 & 0.66\\
                 & \bf Memory (MB) & 0.8 & 0.8 & 1.2 & 1.0 & 1.2 & 2.2 & 4.2 & 7.8 & 15.0  & 29.8\\
  \midrule
  \bf \#Planes 128 & \bf Time(Sec)    & 0.02 & 0.03 & 0.04 & 0.05 & 0.06 & 0.09 & 0.17 & 0.33 & 0.66 & 1.31\\
                 & \bf Memory (MB) & 1.0 & 1.0 & 1.2 & 1.5 & 2.5 & 4.2 & 7.8 & 15.2 & 30.2 & 60\\
  \midrule
  \bf \#Planes 256 & \bf Time(Sec)    & 0.02 & 0.027 & 0.036 & 0.054 & 0.98 & 0.18 & 0.34 & 0.64 & 1.28 & 2.61\\
                 & \bf Memory (MB) & 1.2 & 1.5 & 1.8 & 2.5 & 4.2 & 7.8 & 15.2 & 30.2 & 60.5 & 120.6\\
  \midrule
  \bottomrule
  \end{tabular}

}
\caption{Runtime information about our method, in particular, we show speed and memory usage w.r.t different number of convex polyhedra and hyperplanes.}
\label{tab:nvdiffrec}
\end{table}


==> table/tab4_compactness.tex <==
\begin{table}

\centering
\resizebox{\linewidth}{!}{%
\addtolength{\tabcolsep}{4pt} 
  \begin{tabular}{l ccccc cc cccccc}
  \toprule  
  % \cmidrule(lr){2-5}
  % \cmidrule(lr){6-7}  
  % \cmidrule(lr){8-10}
  % \cmidrule(lr){11-13}
  % \cmidrule(lr){14-15}
  %   \cmidrule(lr){16-17}
   & Plane & Car & Chair & Lamp & Table & Sofa &  Telephone &  Vessel & Loudspeaker & Cabinet & Display & bench & Rifle  \\
  
  \midrule
  \bf \#Vertices & 541.6 & 453.6  & 269.78&548.78 & 188.14&229.74  & 182.62&307.88 &217.18 &190.6 &170.32 &230.92 &410.3\\
  \bf \#Polygons & 300.15 &257.99  & 166.21&305.48 &125.02 & 146.13 & 122.53&185.24 & 139.82&126.51 & 115.87&146.72 &236.76\\
  \bf \#Triangles & 1020.96  & 843.44 & 475.84&1034.52 &313.56 & 396.0 &302.32 &552.32 &370.96 &317.84 &278.32 & 398.48&756.64\\
  \midrule
  % \bf \#GT Vertices & 16275.79 & 36919.14 & 2553.49 & 6944.08& 1160.26 &5917.5 & 3124.05 & 20515.61 & 3986.82 & 1879.29 &1326.28  & 4381.28& 6108.17\\
    \bf \#GT Vertices & 16K & 37K & 2.6K & 7K & 1.1K & 6K & 3.1K & 21K & 4K & 1.9K & 1.3K  & 4.4K& 6.1K\\
  \bottomrule
  \end{tabular}
}
  \caption{Reconstructed mesh property, here we show the average number of vertices, average number of polygons, and average number of triangulated faces of each category.}
\label{tab:nvdiffrec}
\end{table}


==> table/tab5_ablation.tex <==
\begin{table}

\centering
\resizebox{\linewidth}{!}{%
\addtolength{\tabcolsep}{4pt} 
  \begin{tabular}{l ccccc cc cccccc}
  \toprule  
  % \cmidrule(lr){2-5}
  % \cmidrule(lr){6-7}  
  % \cmidrule(lr){8-10}
  % \cmidrule(lr){11-13}
  % \cmidrule(lr){14-15}
  %   \cmidrule(lr){16-17}
   & Plane & Car & Chair & Lamp & Table & Sofa &  Telephone &  Vessel & Loudspeaker & Cabinet & Display & bench & Rifle  \\
  
  \midrule
  \bf \#Vertices & 541.6 & 453.6  & 269.78&548.78 & 188.14&229.74  & 182.62&307.88 &217.18 &190.6 &170.32 &230.92 &410.3\\
  \bf \#Polygons & 300.15 &257.99  & 166.21&305.48 &125.02 & 146.13 & 122.53&185.24 & 139.82&126.51 & 115.87&146.72 &236.76\\
  \bf \#Triangles & 1020.96  & 843.44 & 475.84&1034.52 &313.56 & 396.0 &302.32 &552.32 &370.96 &317.84 &278.32 & 398.48&756.64\\
  \midrule
  % \bf \#GT Vertices & 16275.79 & 36919.14 & 2553.49 & 6944.08& 1160.26 &5917.5 & 3124.05 & 20515.61 & 3986.82 & 1879.29 &1326.28  & 4381.28& 6108.17\\
    \bf \#GT Vertices & 16K & 37K & 2.6K & 7K & 1.1K & 6K & 3.1K & 21K & 4K & 1.9K & 1.3K  & 4.4K& 6.1K\\
  \bottomrule
  \end{tabular}
}
  \caption{Reconstructed mesh property, here we show the average number of vertices, average number of polygons, and average number of triangulated faces of each category.}
\label{tab:nvdiffrec}
\end{table}

